Single-Shot Cuboids: Geodesics-based End-to-end Manhattan Aligned Layout Estimation from Spherical Panoramas

It has been shown that global scene understanding tasks like layout estimation can benefit from wider field of views, and specifically spherical panoramas. While much progress has been made recently, all previous approaches rely on intermediate representations and postprocessing to produce Manhattan-aligned estimates. In this work we show how to estimate full room layouts in a single-shot, eliminating the need for postprocessing. Our work is the first to directly infer Manhattan-aligned outputs. To achieve this, our data-driven model exploits direct coordinate regression and is supervised end-to-end. As a result, we can explicitly add quasi-Manhattan constraints, which set the necessary conditions for a homography-based Manhattan alignment module. Finally, we introduce the geodesic heatmaps and loss and a boundary-aware center of mass calculation that facilitate higher quality keypoint estimation in the spherical domain. Our models and code are publicly available at https://vcl3d.github.io/SingleShotCuboids/.

==> tables/efficiency.tex <==
\begin{table*}[pos=!htbp]
\centering
\caption{
This table presents model complexity measures (multiply-accumulate giga-operations per inference, millions of parameter counts, runtime performance) as well as accuracy (IoU3D) on real domain datasets.
}
\label{tab:efficiency}
\begin{tabular}{@{}cc|cc|cc|r@{}}
\toprule
Method       & Variant      & MACS            & Parameters     & CPU             & GPU             & \multicolumn{1}{l}{IoU3D} \\ \midrule
SSC          & HG-3          & 17.61G          & 6.35M          & 1.78s           & 0.085s          & \textbf{86.02\%}          \\
SSC          & HG-2          & \textbf{12.81G} & \textbf{4.32M} & 1.38s           & 0.058s          & 85.82\%                   \\
LayoutNet v2 & ResNet18    & 76.12G          & 15.57M         & 11.65s          & \textbf{0.034s} & 83.83\%                   \\
LayoutNet v2 & ResNet34    & 95.48G          & 25.68M         & 12.97s          & 0.044s          & 84.60\%                   \\
LayoutNet v2 & ResNet50    & 607.43G         & 91.50M         & 34.63s          & 0.130s          & 82.55\%                   \\
DuLa-Net v2  & ResNet18    & 46.76G          & 25.64M         & 4.99s           & 0.037s          & 83.68\%                   \\
DuLa-Net v2  & ResNet34    & 75.79G          & 45.86M         & 6.46s           & 0.049s          & 84.93\%                   \\
DuLa-Net v2  & ResNet50    & 93.53G          & 57.38M         & 7.22s           & 0.072s          & 85.19\%                   \\
HorizonNet   & ResNet34    & N/A             & N/A            & N/As            & N/A             & 80.43\%                   \\
HorizonNet   & ResNet18    & N/A             & N/A            & N/As            & N/A             & 80.87\%                   \\
HorizonNet   & ResNet50    & 71.70G          & 81.57M         & 3.21s           & 0.063s          & 82.68\%                   \\
CFL          & EfficientNet & 42.19G          & 11.69M         & \textbf{0.420s} & 0.052s          & 78.79\%                   \\ \bottomrule
\end{tabular}
\end{table*}
